AIM: Automatic Interaction Machine for Click-Through Rate Prediction

Feature embedding learning and feature interaction modeling are two crucial components of deep models for Click-Through Rate (CTR) prediction. Most existing deep CTR models suffer from the following three problems. First, feature interactions are either manually designed or simply enumerated. Second, all the feature interactions are modeled with an identical interaction function. Third, in most existing models, different features share the same embedding size which leads to memory inefficiency. To address these three issues mentioned above, we propose Automatic Interaction Machine (AIM) with three core components, namely, Feature Interaction Search (FIS), Interaction Function Search (IFS) and Embedding Dimension Search (EDS), to select significant feature interactions, appropriate interaction functions and necessary embedding dimensions automatically in a unified framework. Specifically, FIS component automatically identifies different orders of essential feature interactions with useless ones pruned; IFS component selects appropriate interaction functions for each individual feature interaction in a learnable way; EDS component automatically searches proper embedding size for each feature. Offline experiments on three large-scale datasets validate the superior performance of AIM. A three-week online A/B test in the recommendation service of a mainstream app market shows that AIM improves DeepFM model by 4.4% in terms of CTR.

==> cover.tex <==
\newpage
\textbf{Cover Letter}

Dear TKDE Editors,

We would like to submit the manuscript, ``AIM: Automatic Interaction Machine for Click-Through Rate Prediction'' to be considered for possible publication on IEEE Transactions on Knowledge and Data Engineering. All authors have checked the manuscript and have agreed to make the submission. We believe the paper may be of particular interest to the readers of your journal. 

Click-through rate (CTR) prediction is a much essential data science task in various online personalization services, including recommender systems, online advertising and web search etc.
Since 2015, deep learning models have become the technique frontier for CTR prediction and achieved state-of-the-art performance.
Feature embedding and feature interaction are two critical components for current deep learning models for CTR prediction. 
However, existing models face three significant downsides: i) Feature interactions are either manually designed or simply enumerated; ii) All feature interactions are modeled with the same specific interaction function but they may need more diverse functions; iii) Different features share the same embedding size to represent their embeddings, which lead to memory inefficiency.
To tackle these issues, we propose \textbf{Automatic Interaction Machine (AIM)} framework with three core components, namely, \textit{Feature Interaction Search (FIS)}, \textit{Interaction Function Search (IFS)} and \textit{Embedding Dimension Search (EDS)}. 
To our knowledge, AIM is the first work that selects significant feature interactions, appropriate IFs and necessary embedding dimensions automatically together. 
Such an automated unified framework enables to largely tapping the potential of deep CTR models.
Extensive experiments on three large-scale real-world datasets and an online A/B test over a commercial platform have demonstrated that our model significantly outperforms the baseline methods.

%The online scenario has been changed, so, the performance is different from the conference version.

A preliminary version of this paper has been presented at the 26th ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining (KDD2020). The differences between conference and journal are significant, as summarized in the difference letter.

We appreciate your time for reviewing this paper and looking forward to receiving any helpful comments! Please feel free to contact with us for any further questions.

Thank you very much for your attention to our paper.

Best Regards,

Chenxu Zhu, Bo Chen, Weinan Zhang, Jincai Lai, Ruiming Tang, Xiuqiang He, Zhenguo Li and Yong Yu

May 23, 2021

\newpage
\textbf{Difference Letter}

Dear TKDE Editors,

A preliminary version of this paper has been published at the 26th ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining (KDD 2020). There are significant differences between this journal submission and the conference version, as summarized in five aspects below.

%There are five major differences between this journal submission and the conference version.
\begin{enumerate}
    \item The model proposed in our conference version only considers to select feature interaction while in our journal version, apart from feature interactions, we search for appropriate interaction functions (IFs) and necessary embedding dimensions in a unified automated framework (Section 3.3, 3.4, 3.5). 
    \item We also add a novel method to introduce high-order feature interactions with quadratically increasing complexity (Section 3.2). We give the specific algorithm and complexity analysis, and this method could be used in AutoFIS and AIM.
    \item We add experiments for AIM, and high-order experiments for both AutoFIS and AIM to demonstrate the effectiveness of AIM and high-order interaction modeling method (Section 4.3). 
    \item We add the effectiveness of selected IFs and selected embedding dimensions (Section 4.4.3 and Section 4.4.4). Besides, we add a comparison between function-wise embedding and shared embedding on AIM and AIM-EDS to validate the effectiveness of EDS and explore the superiority of function-wise embedding (Section 4.4.4). Moreover, we add space and time analysis (Section 4.5) to show the complexity of our model. In addition, we add transferability of AIM to both DeepFM and PNN model (Section 4.6), while in our conference version, we only consider the transferability from AutoFIS to PNN.
    \item We update a new online A/B test on the production version of AIM and witness a significant CTR improvement, 4.4\%, over the production baseline (Section 4.7), which is lower than the conference version due to the changed online scenario. This result demonstrates the magnificent effectiveness of our proposed model.
\end{enumerate}

We believe above differences make this submission of sufficient technical contribution to the community and thus sincerely hope you could consider our submission for publication.

Thank you very much.

Best Regards,

Chenxu Zhu, Bo Chen, Weinan Zhang, Jincai Lai, Ruiming Tang, Xiuqiang He, Zhenguo Li and Yong Yu

May 23, 2021

